Unsupervised Distractor Generation via Large Language Model Distilling and Counterfactual Contrastive Decoding

Within the context of reading comprehension, the task of Distractor Generation (DG) aims to generate several incorrect options to confuse readers. Traditional supervised methods for DG rely heavily on expensive human-annotated distractor labels. In this paper, we propose an unsupervised DG framework, leveraging Large Language Models (LLMs) as cost-effective annotators to enhance the DG capability of smaller student models. Specially, to perform knowledge distilling, we propose a dual task training strategy that integrates pseudo distractors from LLMs and the original answer in-formation as the objective targets with a two-stage training process. Moreover, we devise a counterfactual contrastive decoding mechanism for increasing the distracting capability of the DG model. Experiments show that our unsupervised generation method with Bart-base greatly surpasses GPT-3.5-turbo performance with only 200 times fewer model parameters. Our proposed unsupervised DG method offers a cost-effective framework for practical reading comprehension applications, without the need of laborious distractor annotation and costly large-size models

==> table/intro.tex <==
\begin{table}[tp]
\renewcommand\arraystretch{1.1}
\centering
\small
\begin{tabular}{l|c|c|c}
\hline
 \textbf{Models} & \textbf{Dis 1 B4} & \textbf{Dis 2 B4} & \textbf{Dis 3 B4}\\
\hline
\multicolumn{4}{c}{Finetune} \\
\hline
Bart-base(104M) & 11.22 & 9.83 & 9.15 \\
\hline
\multicolumn{4}{c}{LLM zero-shot inference} \\
\hline
GPT-3.5-turbo(20B) & 6.82 & 5.75 & 5.07 \\
LLaMA-2-13B(13B) & 5.99 & 4.82 & 4.00 \\
\hline
\end{tabular}
[to Figure comparing with our results??]
\caption{Experimental results on dataset RACE. We generate 3 different distractors on Bart-base, GPT-3.5-turbo and LLaMA-2-13B for comparison. B4 refers to BLEU-4 score.}
\label{tab:intro}
\end{table}

==> table/oriCD.tex <==
\begin{table}[tp]
\renewcommand\arraystretch{1.1}
\centering
\small
\begin{tabular}{l|c|c}
\hline
 \textbf{Method} & \textbf{Avg B4}  & \textbf{Avg FS}($\downarrow$)\\
\hline
Ours & 7.64 & 25 \\
Original CD & 1.44 & 39 \\
\hline
\end{tabular}
\caption{Experimental results of original contrastive decoding.}
\label{tab:oriCD}
\end{table}
